Product Line Management with Graphical MBSE Views

Reducing the cost and delay and improving quality are major issues for product and software development, especially in the automotive domain. Product line engineering is a wellknown approach to engineer systems with the aim to reduce costs and development time as well as to improve the product quality. Feature models enable to make logical selection of features and obtain a filtered set of assets that compose the product. We propose to use a color code in feature models to make possible decisions visual in the feature tree. The color code is explained and its use is illustrated. The completeness of the approach is discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{Maurice H. ter Beek and Clemens Dubslaff (Eds.):\\ Proceedings of the First Workshop on Trends\\
in Configurable Systems Analysis (TiCSA'23)\\
EPTCS 392, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.392.4}{10.4204/EPTCS.392.4}}
\pdfoutput=1

